Robust automated calcification meshing for biomechanical cardiac digital twins

Calcification has significant influence over cardiovascular diseases and interventions. Detailed characterization of calcification is thus desired for predictive modeling, but calcified heart meshes for physics-driven simulations are still often reconstructed using manual operations. This poses a major bottleneck for large-scale adoption of computational simulations for research or clinical use. To address this, we propose an end-to-end automated meshing algorithm that enables robust incorporation of patient-specific calcification onto a given heart mesh. The algorithm provides a substantial speed-up from several hours of manual meshing to $\sim$1 minute of automated computation, and it solves an important problem that cannot be addressed with recent template registration-based heart meshing techniques. We validated our final calcified heart meshes with extensive simulations, demonstrating our ability to accurately model patient-specific aortic stenosis and Transcatheter Aortic Valve Replacement. Our method may serve as an important tool for accelerating the development and usage of physics-driven simulations for cardiac digital twins.

==> tables/half_table_example.tex <==
\begin{table}[t!]
\caption{The quantitative effects of our post-processing algorithm on the final calcification mesh. Merged nodes indicate the number of calcification mesh nodes within 1e-2 mm from the heart mesh nodes.}
\centering
\label{table:results_ca2_post_process}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\sisetup{detect-weight,mode=text}
\robustify\bfseries

\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} *{2}{S[table-format=1.3(3),separate-uncertainty=true,table-align-text-post=false]} S[table-format=4.1(3),separate-uncertainty=true,table-figures-uncertainty=1]}
% \begin{tabular*}{\textwidth}{ l @{\extracolsep{\fill}} *{5}{S[table-format=1.2(2),separate-uncertainty=true,table-align-text-post=false]}}

\toprule

{\makecell{Post-process}} & {\makecell{CD (mm)}} & {\makecell{HD 95\% (mm)}} & {\makecell{Merged nodes}} \\

\midrule

None
& 0.000 \pm 0.100 & 0.000 \pm 0.100 & 0.0 \pm 0.1 \\

Ours
& 0.000 \pm 0.100 & 0.000 \pm 0.100 & 0.0 \pm 0.1 \\

\bottomrule

\end{tabular*}

% \begin{flushleft}
% Evaluation of DeepCarve's stitched calcification meshes for all test-set patients. We used the initial calcification segmentation as ground-truth labels and the final stitched meshes as outputs. To convert between the two representations, we used isosurface extraction and voxelization \cite{schroeder1998visualization}. DSC: Dice Similarity Coefficient. Other metrics are similar to previous tables.
% \end{flushleft}

\end{table}

==> tables/table_ca2_seg_postprocess.tex <==
\begin{table*}[t!]
\caption{Segmentation metrics after applying our post-processing algorithm (\FuncCall{PostProcessCa2Seg}) on each representative segmentation prediction model. Same symbols as Table~\ref{table:results_dl_seg}.}
\centering
\label{table:results_ca2_post_process}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\sisetup{detect-weight,mode=text}
\robustify\bfseries

\begin{tabular*}{\linewidth}{ l @{\extracolsep{\fill}} c *{4}{S[table-format=1.3(3),separate-uncertainty=true,table-align-text-post=false]} S[table-format=2.1(4),separate-uncertainty=true,table-figures-uncertainty=1]}
% \begin{tabular*}{\textwidth}{ l @{\extracolsep{\fill}} *{5}{S[table-format=1.2(2),separate-uncertainty=true,table-align-text-post=false]}}

\toprule

\multicolumn{2}{c}{Experiment condition} & \multicolumn{4}{c}{Non-empty target segmentation} & \multicolumn{1}{c}{Empty target} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-7}

{\makecell{Train strategy}} & {\makecell{$I$ minmax}} & {\makecell{Dice \uparrow}} & {\makecell{HD 95\% (mm) \downarrow}} & {\makecell{CD (mm) \downarrow}} & {\makecell{CD_{\textrm{Heart}} \textrm{ (mm)} \downarrow}} & {\makecell{False pos (vx) $\downarrow$}} \\

\midrule
nnU-net    & self-configured &           0.629 \pm 0.158 &           8.315 \pm 10.688 &           1.478 \pm 1.910 & \bfseries 0.929 \pm 0.188 & \bfseries  2.2 \pm  6.4 \\
DiceCE     & [-200, 1500]    &           0.657 \pm 0.086 &           5.058 \pm  7.658 &           0.918 \pm 0.860 &           0.989 \pm 0.219 &           24.9 \pm 41.7 \\
GDL (ours) & [-200, 1500]    & \bfseries 0.657 \pm 0.079 &           5.083 \pm  7.277 & \bfseries 0.834 \pm 0.758 &           0.976 \pm 0.206 &           22.8 \pm 31.0 \\
Gbd        & [-200, 1500]    &           0.632 \pm 0.113 &           4.973 \pm  5.074 &           0.906 \pm 0.644 &           0.979 \pm 0.209 &            2.9 \pm  4.1 \\
Gch        & [-200, 1500]    &           0.624 \pm 0.112 & \bfseries 4.543 \pm  4.421 &           0.900 \pm 0.611 &           0.972 \pm 0.200 &            5.2 \pm  5.4 \\
\midrule

% {\makecell{Train strategy}} & {\makecell{$I$ minmax}} & {\makecell{$\Delta$ Dice \uparrow}} & {\makecell{$\Delta$ HD 95\% (mm) \downarrow}} & {\makecell{$\Delta$ CD (mm) \downarrow}} & {\makecell{$\Delta$ CD_{Heart} (mm) \downarrow}} & {\makecell{$\Delta$ False pos (vx) $\downarrow$}} \\

% nnU-net
% & self-configured & 0.620 \pm 0.224 & 7.015 \pm 8.053 & 1.658 \pm 2.184 & 2.277 \pm 2.293 & 1.3 \pm 2.4  \\

% \midrule

% DiceBCE
% & $[-158, 864]$ & 0.708 \pm 0.190 & 5.580 \pm 8.512 & 1.149 \pm 1.911 & \bfseries 1.047 \pm 0.268 & 21.5 \pm 22.2 \\

% DiceBCE
% & $[-200, 1500]$ & \bfseries 0.719 \pm 0.147 & 5.214 \pm 7.388	 & 1.078 \pm 1.402 & 1.268 \pm 0.703 & \bfseries 20.6 \pm 20.6 \\

% DiceBCE
% & $[-1000, 2500]$ & 0.705 \pm 0.152 & \bfseries 4.587 \pm 6.433 & \bfseries 0.961 \pm 1.305 & 1.089 \pm 0.291 & 115.4 \pm 184.5 \\

% \midrule

% GDL
% & $[-158, 864]$ & 0.714 \pm 0.189 & 5.289 \pm 7.276 & 1.123 \pm 1.707 & 1.086 \pm 0.346 & 36.1 \pm 62.9  \\

% GDL
% & $[-200, 1500]$ & \bfseries 0.737 \pm 0.104 & \bfseries 3.746 \pm 5.426 & \bfseries 0.678 \pm 0.858 & \bfseries 0.994 \pm 0.215 & \bfseries 24.6 \pm 33.1 \\

% GDL
% & $[-1000, 2500]$ & 0.706 \pm 0.157 & 5.896 \pm 7.939 & 1.151 \pm 1.562 & 1.274 \pm 1.030 & 94.1 \pm 124.1 \\

% \midrule

% Gbd
% & $[-200, 1500]$ & \bfseries 0.712 \pm 0.140 & \bfseries 4.174 \pm 5.626 & \bfseries 0.798 \pm 0.811 & \bfseries 0.998 \pm 0.234 & \bfseries 3.8 \pm 4.3 \\

% Gch
% & $[-200, 1500]$ & 0.693 \pm 0.162 & 4.971 \pm 6.724 & 0.907 \pm 0.929 & 1.055 \pm 0.244 & 12.3 \pm 10.3 \\

\end{tabular*}

% \begin{flushleft}
% Evaluation of DeepCarve's stitched calcification meshes for all test-set patients. We used the initial calcification segmentation as ground-truth labels and the final stitched meshes as outputs. To convert between the two representations, we used isosurface extraction and voxelization \cite{schroeder1998visualization}. DSC: Dice Similarity Coefficient. Other metrics are similar to previous tables.
% \end{flushleft}

\end{table*}

==> tables/table_post_process_mesh_metrics.tex <==
\begin{table*}[t!]
\caption{Final tetrahedral calcification mesh metrics with and without our post-processing algorithm. Similar to Table \ref{table:meshing_techniques}, we used 10 repeated trials to obtain these metrics. Spatial accuracy metrics were measured against the ground-truth segmentation. Merged nodes indicate the number of the final calcification mesh nodes within 1e-3 mm from the heart mesh nodes.}
\centering
\label{table:seg_post_process_mesh}

\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\sisetup{detect-weight,mode=text}
\robustify\bfseries

\begin{tabular*}{\linewidth}{ l @{\extracolsep{\fill}} c S[table-format=4(4),separate-uncertainty=true,table-align-text-post=false] *{3}{S[table-format=1.3(3),separate-uncertainty=true,table-align-text-post=false]} S[table-format=2.1(4),separate-uncertainty=true,table-figures-uncertainty=1]}
% \begin{tabular*}{\textwidth}{ l @{\extracolsep{\fill}} *{5}{S[table-format=1.2(2),separate-uncertainty=true,table-align-text-post=false]}}

\toprule

\multicolumn{2}{c}{Experiment condition} & \multicolumn{4}{c}{Non-empty target segmentation} & \multicolumn{1}{c}{Empty target} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-7}

{\makecell{Initial segment}} & {\makecell{Post-process}} & {\makecell{Merged nodes \uparrow}} & {\makecell{Dice \uparrow}} & {\makecell{HD 95\% (mm) \downarrow}} & {\makecell{CD (mm) \downarrow}} & {\makecell{False pos (vx) \downarrow}} \\

\midrule
Ground truth & No  &           2620 \pm 1657 & \bfseries 0.760 \pm 0.039 & \bfseries 1.042 \pm 0.100 & \bfseries 0.321 \pm 0.042 &           N/A \\
Ground truth & Yes & \bfseries 3298 \pm 1907 &           0.671 \pm 0.048 &           1.806 \pm 1.294 &           0.528 \pm 0.139 &           N/A \\
\midrule
GDL (ours)   & No  &           1900 \pm  817 & \bfseries 0.673 \pm 0.084 & \bfseries 3.774 \pm 4.439 & \bfseries 0.794 \pm 0.924 & \bfseries 11.3 \pm 15.2 \\
GDL (ours)   & Yes & \bfseries 2686 \pm 1101 &           0.621 \pm 0.081 &           5.281 \pm 7.178 &           0.913 \pm 0.737 &           18.1 \pm 23.9 \\
\bottomrule

\end{tabular*}

\end{table*}
